Explicit Modelling of Physical Measures: From Event-B to Java

The increasing development of cyber-physical systems (CPSs) requires modellers to represent and reason about physical values. This paper addresses two major, inter-related, aspects that arise when modelling physical measures. Firstly, there is often a heterogeneity of representation; for example: speed can be represented in many different units (mph, kph, mps, etc. . . ). Secondly, there is incoherence in composition; for example: adding a speed to a temperature would provide a meaningless result in the physical world, even though such a purely mathematical operation is meaningful in the abstract. These aspects are problematic when implicit semantics - concerned with measurements - in CPSs are not explicit (enough) in the requirements, design and implementation models. We present an engineering approach for explicitly modelling measurements during all phases of formal system development. We illustrate this by moving from Event-B models to Java implementations, via object oriented design.

==> eptcsdata.tex <==
\providecommand{\firstpage}{64}
\providecommand{\publicationstatus}{R. Laleau, D. M\'ery, S. Nakajima, E. Troubitsyna (Eds): Joint Workshop on\\ Handling IMPlicit and EXplicit knowledge in formal system development\\ and  Formal \& Model-Driven Techniques for Developing Trustworthy Systems.\\
EPTCS 271, 2018, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.271.5}{10.4204/EPTCS.271.5}}
\pdfoutput=1

